On a triply graded Khovanov homology

Cobordisms are naturally bigraded and we show that this grading extends to Khovanov homology, making it a triply graded theory. Although the new grading does not make the homology a stronger invariant, it can be used to show that odd Khovanov homology is multiplicative with respect to disjoint unions and connected sums of links; same results hold for the generalized Khovanov homology defined by the author in his previous work. We also examine the module structure on both odd and even Khovanov homology, in particular computing the effect of sliding a basepoint through a crossing on the integral homology.

==> images/pics-tangles.tex <==
%\newlength\fntinkwidth
%\newlength\fntsize
%\newlength\fntshift
%\newbox\fntbox

\makeatletter

%% \defPicFonts{family}{name}(x0,y0)(x1,y1):size:<size_factor>[r|c|<empty>|outline_code]{code}

\def\defPicFonts#1#2{\@ifnextchar(%
	{\defPicFonts@getcoords{#1}{#2}}%
	{\defPicFonts@getsize{#1}{#2}(-0.5,-0.5)(0.5,0.5)}}
	
\def\defPicFonts@getcoords#1#2(#3){\@ifnextchar(%
	{\defPicFonts@getsize{#1}{#2}(#3)}%
	{\defPicFonts@getsize{#1}{#2}(0,0)(#3)}}

\def\defPicFonts@getsize#1#2(#3)(#4){\@ifnextchar:%)
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}}%
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}:W:}}
	
\def\defPicFonts@getsizefactor#1#2#3:#4:{\@ifnextchar<%>
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}}%
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}<1>}}

\def\defPicFonts@getoutline#1#2#3#4<#5>{\@ifnextchar[%]
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}}%
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}[]}}

\def\defPicFonts@getcode#1#2#3#4#5[#6]#7{%
	\ifx#6r\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\psframe[linewidth=0.3pt,linestyle=dotted]#3}{#7}%
	\else\ifx#6c\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\pscircle[linewidth=0.3pt,linestyle=dotted](0,0){0.5}}{#7}%
	\else
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{#6}{#7}%
	\fi\fi
}

%% \defPicFonts@define{family}{name}{coords}{hbox_for_size}{size_factor}{outline_code}{code}
%%
\def\defPicFonts@define#1#2#3#4#5#6#7{%
	%
	%	#1#2 draws the symbol using PS-Tricks unit
	% starred version: with outline
	\expandafter\edef\csname#1#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname#1#2@draw\endcsname##1##2{\begingroup
		\pspicture#3%
			\psset{linewidth=0.5pt,dotsep=1pt,arrowsize=5pt,arrowlength=1}%
			##1#6##2#7%
		\endpspicture\endgroup}%
	%
	% fnt#1#2 draws the symbol as a font
	% starred version: no outline
	\expandafter\edef\csname fnt#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname fnt#2@size\endcsname##1##2{%
		\def\fnt@drawcode{#7##1#6##2}%
		\ifmmode
			\edef\next{\noexpand\mathchoice
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\displaystyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptfont\noexpand\scriptstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptscriptfont\noexpand\scriptscriptstyle}}%
		\else
			\edef\next{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
		\fi
		\next
	}
	\expandafter\def\csname fnt#2@draw\endcsname##1##2{\begingroup
		\fntinkwidth=\fontdimen8##13\relax
		\setbox\fntbox=\hbox{$\m@th##2#4$}%
		\fntshift= \dp\fntbox	\fntshift=#5\fntshift
		\fntsize = \ht\fntbox	\fntsize=#5\fntsize	\advance\fntsize\fntshift
		\psset{unit=\fntsize,linewidth=\fntinkwidth,dotsep=1pt,arrowsize=7\pslinewidth,arrowlength=0.8,arrowinset=0.6}%
		\hskip\fntinkwidth\ifmmode
			\vcenter{\hbox{\pspicture#3\fnt@drawcode\endpspicture}}%
		\else
			\pspicture[shift=-\fntshift]#3\fnt@drawcode\endpspicture
		\fi\hskip\fntinkwidth
	\endgroup}
}

\makeatother

%%
%%	Crossings and resolutions
%%
\defPicFonts{big}{Circle}:|:{\pscircle[linewidth=0.5pt](0,0.05){0.45}}

\defPicFonts{big}{NWSECr}[r]{%
		\psline(-0.5,-0.5)(0.5,0.5)
		\psline[border=3\pslinewidth](-0.5,0.5)(0.5,-0.5)
}%

\defPicFonts{big}{NESWCr}[r]{%
		\psline(-0.5,0.5)(0.5,-0.5)
		\psline[border=3\pslinewidth](-0.5,-0.5)(0.5,0.5)
}%

\defPicFonts{big}{VertRes}[r]{%
		\psbezier(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.5,0.5)
		\psbezier( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.5,0.5)
}%

\defPicFonts{big}{HorRes}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
}%

\defPicFonts{big}{HorResCob}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
		\psline[linewidth=3\pslinewidth](0,-0.18)(0,0.18)
}%

\defPicFonts{big}{PosCr}[r]{%
		\psline{->}(0.5,-0.5)(-0.55,0.55)
		\psline[border=3\pslinewidth]{->}(-0.5,-0.5)(0.55,0.55)
}%

\defPicFonts{big}{NegCr}[r]{%
		\psline{->}(-0.5,-0.5)(0.55,0.55)
		\psline[border=3\pslinewidth]{->}(0.5,-0.5)(-0.55,0.55)
}%

\defPicFonts{big}{NoCr}[r]{%
		\psbezier{->}(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.55,0.55)
		\psbezier{->}( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.55,0.55)
}%

\defPicFonts{big}{PosCrArrowUp}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{->}(0,-0.5)(0,0.7)
}%

\defPicFonts{big}{PosCrArrowDown}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{<-}(0,-0.7)(0,0.5)
}%

%%
%%	A horizontal full twist tangle
%%
\defPicFonts{tangle}{FullTwist}:|:<1.25>[c]{%
	\psclip{\psframe[linestyle=none](0,-1)(1,1)}
		\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
	\psclip{\psframe[linestyle=none](0.1,-1)(-1,1)}
		\psbezier[border=3\pslinewidth](-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
}

%%
%%	Twisted unknots
%%
\defPicFonts{tangle}{PosTwist}(-1,-0.5)(1,0.5)[r]{%
	\psbezier{C-C}( 0.5,-0.5)( 0.2,-0.5)(-0.2,0.5)(-0.5,0.5)
	\psbezier[border=3\pslinewidth]{C-C}(-0.5,-0.5)(-0.2,-0.5)( 0.2,0.5)( 0.5,0.5)
	\psarc{C-C}(-0.5,0){0.5}{90}{270}%
	\psarc{C-C}(0.5,0){0.5}{-90}{90}%
}

\defPicFonts{tangle}{PosTwistHor}(-1,-0.5)(1,0.5)[r]{\pscustom{%
	\moveto(-0.5,0.5)
	\psarc(-0.5,0){0.5}{90}{270}\curveto(-0.3,-0.5)(-0.2,-0.2)(0,-0.2)\curveto( 0.2,-0.2)( 0.3,-0.5)( 0.5,-0.5)
	\psarc( 0.5,0){0.5}{-90}{90}\curveto( 0.3, 0.5)( 0.2, 0.2)(0, 0.2)\curveto(-0.2, 0.2)(-0.3, 0.5)(-0.5, 0.5)
	\stroke
}}

\defPicFonts{tangle}{PosTwistVert}(-1,-0.5)(1,0.5)[r]{%
	\psarc{C-C}( 0.5,0){0.5}{-90}{90}\psellipticarc{C-C}( 0.5,0)(0.4,0.5){90}{270}%
	\psarc{C-C}(-0.5,0){0.5}{90}{270}\psellipticarc{C-C}(-0.5,0)(0.4,0.5){-90}{90}%
}

%%
%%	First Reidemeister move
%%
\defPicFonts{tangle}{RIline}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(0, 0.2)(0,0)
	\psbezier(-0.35355,-0.35355)(-0.25355,-0.15355)(0,-0.2)(0,0)
}

\defPicFonts{tangle}{RIx}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(-0.1,-0.2)(0.1,-0.2)
	\psbezier[border=3\pslinewidth](-0.35355,-0.35355)(-0.25355,-0.15355)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
}
	
\defPicFonts{tangle}{RIh}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2, 0)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
	\psbezier(-0.35355,-0.35355)(-0.2, 0)(-0.1,-0.2)(0.1,-0.2)
}

\defPicFonts{tangle}{RIv}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
}

\defPicFonts{tangle}{RIcob}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
	\psline[linewidth=3\pslinewidth](-0.24,0)(-0.1,0)
}

%%
%%	Second Reidemeister move
%%
\defPicFonts{tangle}{RIIxx}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhh}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIhv}:|:<1.25>[c]{%
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
	\psarc(0,0){0.2}{-90}{90}
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvh}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\psarc(0,0){0.2}{90}{270}
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvv}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\pscircle(0,0){0.2}
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhhs}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.2,0)(0.2,0)(0.433, 0.25)
	\psbezier(-0.433,-0.25)(-0.2,0)(0.2,0)(0.433,-0.25)
}

%%
%%	Third Reidemeister move
%%
\defPicFonts{tangle}{RIIIax}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIah}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIav}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIac}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIahhh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psarc(0,0.2){0.15}{45}{315}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahhv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\pscircle(0,0.2){0.15}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psarc(0,0.2){0.15}{45}{135}
	\psarc(0,0.2){0.15}{225}{315}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psarc(0,0.2){0.15}{-135}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{225}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{225}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{135}
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIbx}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbc}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

%%
%%	Three horizontal lines
%%
\defPicFonts{tangle}{IIIVert}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
}

\defPicFonts{tangle}{IIIVertT}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,0.14839)
}

\defPicFonts{tangle}{IIIVertB}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,-0.14839)
}

%%
%%	Passing a circle over a link
%%
\defPicFonts{tangle}{CircLeft}(-0.75,-1)(1,1):|:<0.625>[r]{%
	\psline(0.75,-1)(0.75,1)
	\pscircle(0,0){0.5}
}
\defPicFonts{tangle}{CircRight}(-1,-1)(0.75,1):|:<0.625>[r]{%
	\psline(-0.75,-1)(-0.75,1)
	\pscircle(0,0){0.5}
}
\defPicFonts{tangle}{CircOver}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\psline(0,-1)(0,1)
	\pscircle[border=3\pslinewidth](0,0){0.5}
}
\defPicFonts{tangle}{CircUnder}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\pscircle(0,0){0.5}
	\psline[border=3\pslinewidth](0,-1)(0,1)
}

\defPicFonts{tangle}{CircOverhh}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\pscustom{\moveto(0,-1)
		\curveto( 0  ,-0.25)( 0.5,-0.4 )( 0.5,0)
		\curveto( 0.5, 0.4 )( 0.2, 0.6 )( 0  ,0)
		\curveto(-0.2,-0.6 )(-0.5,-0.4 )(-0.5,0)
		\curveto(-0.5, 0.4 )( 0  , 0.25)( 0  ,1)
		\stroke
	}
}
\defPicFonts{tangle}{CircOverhv}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\pscustom{\moveto(0,-1)
		\curveto(0  ,-0.25)(0.5,-0.4 )(0.5,0)
		\curveto(0.5, 0.4 )(0  , 0.25)(0  ,1)
		\stroke}%
	\pscustom{\moveto(0,0)
		\curveto( 0  ,-0.6)(-0.5,-0.4)(-0.5,0)
		\curveto(-0.5, 0.4)( 0  , 0.6)( 0  ,0)
		\stroke}%
}
\defPicFonts{tangle}{CircOvervh}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\pscustom{\moveto(0,-1)
		\curveto( 0  ,-0.25)(-0.5,-0.4 )(-0.5,0)
		\curveto(-0.5, 0.4 )( 0  , 0.25)( 0  ,1)
		\stroke}%
	\pscustom{\moveto(0,0)
		\curveto(0  ,-0.6)(0.5,-0.4)(0.5,0)
		\curveto(0.5, 0.4)(0  , 0.6)(0  ,0)
		\stroke}%
}
\defPicFonts{tangle}{CircOvervv}(-0.75,-1)(0.75,1):|:<0.625>[r]{%
	\pscustom{\moveto(0,-1)
		\curveto( 0  ,-0.25)(-0.5,-0.4 )(-0.5,0)
		\curveto(-0.5, 0.4 )(-0.2, 0.6 )( 0  ,0)
		\curveto( 0.2,-0.6 )( 0.5,-0.4 )( 0.5,0)
		\curveto( 0.5, 0.4 )( 0  , 0.25)( 0  ,1)
		\stroke
	}
}


==> images/relations.tex <==
\def\pictRelS{\begin{centerpict}(0,0)(1,1)
	\psset{linewidth=0.5pt,dash=1pt 1.5pt,dimen=middle}
	\pscircle(0.5,0.5){0.4}
	\psellipticarc[linewidth=0.5\pslinewidth](0.5,0.5)(0.4,0.15){180}{360}
	\psellipticarc[linewidth=0.5\pslinewidth,linestyle=dashed](0.5,0.5)(0.4,0.15){0}{180}
\end{centerpict}}

\def\pictRelT{\begin{centerpict}(-0.5,-0.7)(0.5,0.7)
	\psset{linewidth=0.5pt,dash=1pt 1.5pt,dimen=middle}
	\psellipse(0,0)(0.45,0.6)
	\psellipticarc(0.3,0)(0.4,0.45){130}{230}
	\psclip{\psellipse[linestyle=none](0.3,0)(0.4,0.45)}
		\psellipticarc(-0.3,0)(0.4,0.45){-50}{50}
	\endpsclip
	\psellipticarc[linewidth=0.5\pslinewidth](0.275,0)(0.175,0.075){180}{360}
	\psellipticarc[linewidth=0.5\pslinewidth](-0.275,0)(0.175,0.075){180}{360}
	\psellipticarc[linewidth=0.5\pslinewidth,linestyle=dashed](0.275,0)(0.175,0.075){0}{180}
	\psellipticarc[linewidth=0.5\pslinewidth,linestyle=dashed](-0.275,0)(0.175,0.075){0}{180}
\end{centerpict}}

\def\pictRelTuCircles{%
	\psset{linewidth=0.5pt,dash=1pt 1.5pt,dimen=middle}
	\psellipticarc(0.2,0.1)(0.2,0.07\psxunit){-180}{0}
	\psellipticarc(1.0,0.1)(0.2,0.07\psxunit){-180}{0}
	\psellipticarc[linewidth=0.5\pslinewidth,linestyle=dashed](0.2,0.1)(0.2,0.07\psxunit){0}{180}
	\psellipticarc[linewidth=0.5\pslinewidth,linestyle=dashed](1.0,0.1)(0.2,0.07\psxunit){0}{180}
	\psellipse(0.2,1.4)(0.2,0.07\psxunit)
	\psellipse(1.0,1.4)(0.2,0.07\psxunit)
}

\def\pictRelTuL{\begin{centerpict}(-0.1,0)(1.3,1.5)
	\pictRelTuCircles
	\psline(0.0,0.1)(0.0,1.4)\psline(0.4,0.1)(0.4,1.4)
	\psbezier(0.8,0.1)(0.8,0.7)(1.2,0.7)(1.2,0.1)
	\psbezier(0.8,1.4)(0.8,0.8)(1.2,0.8)(1.2,1.4)
\end{centerpict}}

\def\pictRelTuR{\begin{centerpict}(-0.1,0)(1.3,1.5)
	\pictRelTuCircles
	\psbezier(0.0,0.1)(0.0,0.7)(0.4,0.7)(0.4,0.1)
	\psbezier(0.0,1.4)(0.0,0.8)(0.4,0.8)(0.4,1.4)
	\psline(0.8,0.1)(0.8,1.4)\psline(1.2,0.1)(1.2,1.4)
\end{centerpict}}

\def\pictRelTuB{\begin{centerpict}(-0.1,0)(1.3,1.5)
	\pictRelTuCircles
	\psbezier(0.0,0.1)(0.0,1.0)(1.2,1.0)(1.2,0.1)
	\psbezier(0.4,0.1)(0.35,0.5)(0.85,0.5)(0.8,0.1)
	\psbezier(0.0,1.4)(0.0,1.0)(0.4,1.0)(0.4,1.4)
	\psbezier(0.8,1.4)(0.8,0.8)(1.2,0.8)(1.2,1.4)
\end{centerpict}}

\def\pictRelTuT{\begin{centerpict}(-0.1,0)(1.3,1.5)
	\pictRelTuCircles
	\psbezier(0.0,1.4)(0.0,0.5)(1.2,0.5)(1.2,1.4)
	\psbezier(0.4,1.4)(0.35,1.0)(0.85,1.0)(0.8,1.4)
	\psbezier(0.0,0.1)(0.0,0.5)(0.4,0.5)(0.4,0.1)
	\psbezier(0.8,0.1)(0.8,0.7)(1.2,0.7)(1.2,0.1)
\end{centerpict}}



==> khovanov-pict.tex <==
\begingroup
\psset{unit=1cm}
\def\cobordism{%
	\rput(0,0){\psclip{\pscustom[linestyle=none]{%
			\moveto(-1.40851, 0.73936)
			\lineto(-0.97994, 0.73936)
			\lineto(-0.97994, 0.00325)
			\lineto( 0.41979,-0.52933)
			\curveto(0.41979, 0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
			\lineto( 1.66534,-0.49630)
			\lineto( 1.66534, 1)
			\lineto(-1.40851, 1)}}
		\psset{linestyle=dashed,dash=1pt 1.5pt,linewidth=0.15pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.35)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=dashed,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.64296,-0.64475)(0.14597,-0.58989)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.81076,-0.42482)(0.65569,-0.168)
	\endpsclip}
	\rput(0,0){\psclip{\pscustom[linestyle=none]{%
			\moveto(-1.40851, 0.73936)
			\lineto(-0.97994, 0.73936)
			\lineto(-0.97994, 0.00325)
			\lineto( 0.41979,-0.52933)
			\curveto(0.41979, 0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
			\lineto( 1.66534,-0.49630)
			\lineto( 1.8,-0.49630)
			\lineto( 1.8,-1)
			\lineto(-1.6,-1)
			\lineto(-1.6, 0.73936)}}
		\psset{linestyle=solid,linewidth=0.5pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.32)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=solid,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.64296,-0.64475)(0.14597,-0.58989)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.81076,-0.42482)(0.65569,-0.168)
	\endpsclip}
	\rput(0,1.5){%
		\psset{linestyle=solid,linewidth=0.5pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.32)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=solid,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.81076,-0.42482)(0.65569,-0.168)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.44416,-0.62280)(0.14597,-0.58989)
	}
	\rput(0,0){%
		\psset{linewidth=0.5pt,dash=1pt 1.5pt}
		\psline{c-c}(-1.40851, 0.73936)(-1.40851,2.25000)
		\psline{c-c}(-0.97994, 0.00325)(-0.97994,1.50325)
		\psdash\psline{c-c}( 0.08996, 0.31025)( 0.08996,1.221)
		\psdash\psline{c-c}( 0.39409, 0.14265)( 0.39409,1.14265)
		\psline{-c}( 0.08996, 1.221)( 0.08996,1.81025)
		\psline{-c}( 0.39409, 1.14265)( 0.39409,1.64265)
		\psline{c-c}( 1.66534,-0.49630)( 1.66534,1.00370)
		\psbezier{c-c}( 0.41979,-0.52933)( 0.41979,0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
		\rput(0.58652,0.2782){\psline[linewidth=0.3pt,arrowsize=4pt,arrowlength=1]{->}(0.1,0.1)(-0.4,-0.05)}
	}
}

\def\cubevertex#1#2#3{\begingroup
	\psset{linewidth=0.8pt,linestyle=solid}%
	\begin{pspicture}(-1,-0.8)(1,1.1)%
		\pspolygon[fillcolor=white,fillstyle=solid,linestyle=none](-1,-0.8)(1,-0.8)(1,1.2)(-1,1.2)
		\trefoilresolution{#1}{#2}{#3}%
		\rput*[t](0,-0.85){\small $#1#2#3$}%
	\end{pspicture}%
\endgroup}

\def\cubeedge#1#2#3{\begingroup
	\psset{linewidth=0.5pt,linestyle=solid,unit=0.5}%
	\begin{centerpict}(-0.8,-0.7)(0.8,1)%
		\trefoilresolution{#1}{#2}{#3}%
	\end{centerpict}%
\endgroup}

\begin{pspicture}(0,0)(16.5,13)
%	\pspolygon[linewidth=1pt,linestyle=dotted,linecolor=blue](0,0)(16.5,0)(16.5,13)(0,13)
	% Top left corner: knot diagram
	\rput[tl](0,13){$\left\llbracket\trefoil aca\right\rrbracket$}
	% Bottom: chain complex
	\rput( 2.1, 0.5){\Rnode[href=-0.25]{C0}{\Large $C^0$}}
	\rput( 6.4, 0.5){\Rnode[href=-0.25]{C1}{\Large $C^1$}}
	\rput(10.7, 0.5){\Rnode[href=-0.25]{C2}{\Large $C^2$}}
	\rput(15.0, 0.5){\Rnode[href=-0.25]{C3}{\Large $C^3$}}
	\begingroup
	\psset{linestyle=solid,linewidth=1pt,nodesep=3pt,arrowsize=4.5pt}
	\ncline{->}{C0}{C1}	\naput{$d$}
	\ncline{->}{C1}{C2}	\naput{$d$}
	\ncline{->}{C2}{C3}	\naput{$d$}
	\endgroup
	% Vertical dotted lines --- direct sum
	\pnode( 2.0, 8){col0}
	\pnode( 6.3,12){col1}
	\pnode(10.6,12){col2}
	\pnode(14.9, 8){col3}
	\begingroup
	\psset{linestyle=dotted,linewidth=1pt,nodesep=3pt,arrowsize=5pt}
	\ncline{->}{col0}{C0}
	\ncline{->}{col1}{C1}	%\uput[r]( 6.3,1.7){$\cdot\,\{1\}$}
	\ncline{->}{col2}{C2}	%\uput[r](10.6,1.7){$\cdot\,\{2\}$}
	\ncline{->}{col3}{C3}	%\uput[r](14.9,1.7){$\cdot\,\{3\}$}
	\endgroup
	% Resolutions
	\rput( 2.0, 8){\rnode{000}{\cubevertex{0}{0}{0}}}
	\rput( 6.3,12){\rnode{100}{\cubevertex{1}{0}{0}}}
	\rput( 6.3, 8){\rnode{010}{\cubevertex{0}{1}{0}}}
	\rput( 6.3, 4){\rnode{001}{\cubevertex{0}{0}{1}}}
	\rput(10.6,12){\rnode{110}{\cubevertex{1}{1}{0}}}
	\rput(10.6, 8){\rnode{101}{\cubevertex{1}{0}{1}}}
	\rput(10.6, 4){\rnode{011}{\cubevertex{0}{1}{1}}}
	\rput(14.9, 8){\rnode{111}{\cubevertex{1}{1}{1}}}
	\begingroup
	\psset{linestyle=solid,linewidth=1pt,nodesep=-2pt,labelsep=1pt,arrowsize=5pt}
	\ncline{->}{000}{100}		\nbput{$\scriptstyle {*}00$}	\naput{\cubeedge{a}{0}{0}}
	\ncline{->}{000}{010}		\nbput{$\scriptstyle 0{*}0$}	\naput{\cubeedge{0}{c}{0}}
	\ncline{->}{000}{001}		\nbput{$\scriptstyle 00{*}$}	\naput{\cubeedge{0}{0}{a}}
	\ncline{->}{010}{110}	\nbput[npos=0.15]{$\scriptstyle {*}10$}
												\naput[npos=0.12]{$-\permMM$\cubeedge{a}{1}{0}}
	\ncline{->}{010}{011}	\naput[npos=0.20]{$\scriptstyle 01{*}$}
												\naput[npos=0.85]{$\!\!\!\!\!\!\!-\permMM$\cubeedge{0}{1}{a}}
	\ncline{->}{100}{110}	\nbput[npos=0.50]{$\scriptstyle 1{*}0$}
												\naput{\cubeedge{1}{c}{0}}
	\ncline[border=2pt]{->}{100}{101}	\naput[npos=0.20]{$\scriptstyle 10{*}$}
																		\naput[npos=0.80]{\cubeedge{1}{0}{a}}
	\ncline[border=2pt]{->}{001}{101}	\nbput[npos=0.15]{$\scriptstyle {*}01$}
																		\naput[npos=0.15]{$-\permMM$\cubeedge{a}{0}{1}}
	\ncline{->}{001}{011}	\naput{$\scriptstyle 0{*}1$}
												\nbput{\cubeedge{0}{c}{1}}
	\ncline{->}{110}{111}	\nbput[npos=0.5]{$\scriptstyle 11{*}$}
												\naput{\cubeedge{1}{1}{a}}
	\ncline{->}{101}{111}	\nbput[npos=0.5]{$\scriptstyle 1{*}1$}
												\naput[npos=0.35]{$-\permMM$\cubeedge{1}{c}{1}}
	\ncline{->}{011}{111}	\naput[npos=0.5]{$\scriptstyle {*}11$}
												\nbput{$\!\!\!\!-\permSS$\cubeedge{a}{1}{1}}
	\endgroup
	%% cobordism
	\rput(1.5,3){\begingroup
		\psframe[linestyle=none,fillstyle=solid,fillcolor=white](0.3,-0.6)(0.7,1.5)
		\psset{yunit=0.64,xunit=0.8}
		\cobordism
	\endgroup}
	\pscurve[border=1pt,linewidth=0.3pt,arrowsize=4pt]{->}(4.15,7.5)(4,7)(3,6)(2.7,5.5)(2.2,4.3)
\end{pspicture}
\endgroup

